Measurements of $\pi^{\pm}$ differential yields from the surface of the T2K replica target for incoming 31 GeV/c protons with the NA61/SHINE spectrometer at the CERN SPS

Measurements of particle emission from a replica of the T2K 90 cm-long carbon target were performed in the NA61/SHINE experiment at CERN SPS, using data collected during a high-statistics run in 2009. An efficient use of the long-target measurements for neutrino flux predictions in T2K requires dedicated reconstruction and analysis techniques. Fully-corrected differential yields of $\pi^\pm$-mesons from the surface of the T2K replica target for incoming 31 GeV/c protons are presented. A possible strategy to implement these results into the T2K neutrino beam predictions is discussed and the propagation of the uncertainties of these results to the final neutrino flux is performed.

==> pion_numerical_tables.tex <==
\section{Numerical Tables}\label{chap:NumericalTables}

Numerical results for the article 
``Measurements of $\pi^\pm$ differential yields from the surface of the 
T2K replica target for incoming 31~GeV/$c$ protons with the NA61/SHINE 
spectrometer at the CERN SPS'' arXiv:1603.06774 [hep-ex].

Fully-corrected differential yields of $\pi^+$-mesons (Table 1) and
$\pi^-$-mesons (Table 2) from the surface of 
the T2K replica target per incoming 31~GeV/$c$ protons. 
The yields with statistical and systematic uncertainties
are given in $(z, \theta, p)$ bins.

%Table 1 shows numerical values of multiplicity of positively charged pions per incident 31~GeV/$c$ proton on the T2K replica target produced in $(p,\theta,z)$ bins with statistical and systematic uncertainties.

%Table 2 shows the numerical values of the negatively charged pion multiplicities for each $(p,\theta,z)$ bins with the related statistical and systematic uncertainties.

\clearpage
\newpage

\pgfplotstableset{
begin table=\begin{longtable},
end table=\end{longtable},
%begin table=\begin{supertabular},
%end table=\end{supertabular},
}

\pgfplotstabletypeset[
%every nth row={115}{before row=\hline},
%every last row/.style={before row=\hline, after row=\hline},
every head row/.style={before row=\caption{Yields of $\pi^{+}$ in $(z, \theta, p)$ bins with statistical and systematic uncertainties}\\\toprule, after row=\midrule\endhead}, 
every last row/.style={after row=\bottomrule},
col sep=tab,
string type,
columns/z/.style={column name=\textbf{$z$}, column type={c}},
columns/theta/.style={column name=\begin{tabular}[t]{@{}c@{}}\textbf{$\theta$}\\$[$mrad$]$\end{tabular}, column type={c}},
%columns/plow/.style={column name=\textbf{}, column type={r}, fixed, fixed zerofill, dec sep align, precision=3},
columns/p/.style={column type=p{0.05\linewidth},column name=\begin{tabular}[t]{@{}c@{}}\textbf{$p$}\\$[$GeV/$c]$\end{tabular}, column type={c}},
%columns/phigh/.style={column name=\textbf{}, column type={l}, fixed, fixed zerofill, dec sep align, precision=3},
columns/multiplicities/.style={column type=p{0.3\linewidth},column name=\begin{tabular}[t]{@{}c@{}}\textbf{dn/dp$\times$1/p.o.t.}\\$[$1/(GeV/$c$)$]$\end{tabular}, column type={c}, sci, sci zerofill, sci sep align, precision=3, sci 10e},
columns/Stat/.style={column name=\begin{tabular}[t]{@{}c@{}}\textbf{$\Delta_{stat}$}\\$[$1/(GeV/$c$)$]$\end{tabular}, column type={c}, sci, sci zerofill, sci sep align, precision=3, sci 10e},
columns/StatFrac/.style={column name=\textbf{$\Delta_{stat}$ (frac)}, column type={c}, fixed, fixed zerofill, dec sep align, precision=3},
columns/Sys/.style={column name=\begin{tabular}[t]{@{}c@{}}\textbf{$\Delta_{sys}$}\\$[$1/(GeV/$c$)$]$\end{tabular}, column type={c}, sci, sci zerofill, sci sep align, precision=3, sci 10e},
columns/SysFrac/.style={column name=\textbf{$\Delta_{sys}$ (frac)}, column type={c}, fixed, fixed zerofill, dec sep align, precision=3},
]{./na61_piplus_replica_2009_paper.txt}

\clearpage
\newpage


\pgfplotstableset{
begin table=\begin{longtable},
end table=\end{longtable},
%begin table=\begin{supertabular},
%end table=\end{supertabular},
}

\pgfplotstabletypeset[
%every nth row={115}{before row=\hline},
%every last row/.style={before row=\hline, after row=\hline},
every head row/.style={before row=\caption{Yields of $\pi^{-}$ in $(z, \theta, p)$ bins with statistical and systematic uncertainties}\\\toprule, after row=\midrule\endhead}, 
every last row/.style={after row=\bottomrule},
col sep=tab,
string type,
columns/z/.style={column name=\textbf{$z$}, column type={c}},
columns/theta/.style={column name=\begin{tabular}[t]{@{}c@{}}\textbf{$\theta$}\\$[$mrad$]$\end{tabular}, column type={c}},
%columns/plow/.style={column name=\textbf{}, column type={r}, fixed, fixed zerofill, dec sep align, precision=3},
columns/p/.style={column type=p{0.05\linewidth},column name=\begin{tabular}[t]{@{}c@{}}\textbf{p}\\$[$GeV/$c]$\end{tabular}, column type={c}},
%columns/phigh/.style={column name=\textbf{}, column type={l}, fixed, fixed zerofill, dec sep align, precision=3},
columns/multiplicities/.style={column type=p{0.3\linewidth},column name=\begin{tabular}[t]{@{}c@{}}\textbf{dn/dp$\times$1/p.o.t.}\\$[$/(GeV/c)/p.o.t$]$\end{tabular}, column type={c}, sci, sci zerofill, sci sep align, precision=3, sci 10e},
columns/Stat/.style={column name=\begin{tabular}[t]{@{}c@{}}\textbf{$\Delta_{stat}$}\\$[$1/(GeV/$c$)$]$\end{tabular}, column type={c}, sci, sci zerofill, sci sep align, precision=3, sci 10e},
columns/StatFrac/.style={column name=\textbf{$\Delta_{stat}$ (frac)}, column type={c}, fixed, fixed zerofill, dec sep align, precision=3},
columns/Sys/.style={column name=\begin{tabular}[t]{@{}c@{}}\textbf{$\Delta_{sys}$}\\$[$1/(GeV/$c$)$]$\end{tabular}, column type={c}, sci, sci zerofill, sci sep align, precision=3, sci 10e},
columns/SysFrac/.style={column name=\textbf{$\Delta_{sys}$ (frac)}, column type={c}, fixed, fixed zerofill, dec sep align, precision=3},
]{./na61_piminus_replica_2009_paper.txt}




